Chiral Effective Field Theories for Strong and Weak Dynamics

The chiral effective field theory (ChEFT) is an extension of the chiral perturbation theory that includes the nuclear forces and weak currents at the hadronic and nuclear scales. We propose a systematic framework of parametrising the pion-nucleon and nucleon-nucleon Lagrangian via the Weinberg power counting rules. We enumerate the operator bases of ChEFT by extending the Hilbert series of the pure meson sector to the nucleon sector with the CP symmetries. The Young tensor method is utilized to obtain the complete sets of the nucleon-nucleon, three-nucleon operators with/without pions ($\not\pi$-EFT). Then we use the spurion technique to reconstruct the ChEFT Lagrangian by taking the adjoint spurion and leptonic fields as the building blocks, without the need of external sources. These operators can be applied to both the strong dynamics, and the nucleon/nuclear weak current processes.

==> sec-app2.tex <==
\section{Comparison to Literature}
\label{sec:app2}



Many authors have been working on the ChEFT. In this appendix we will make a comparison to the previous literature.

\subsection*{Meson-Nucleon sector}

The reference~\cite{Fettes:2000gb} constructed the effective operators up to $\mathcal{O}(q^4)$, but via a different method. In this section, we will summarize the method used in Ref.~\cite{Fettes:2000gb} and show the difference between their result from ours.  

The methodology of Ref.~\cite{Fettes:2000gb} is to separate the meson factor out in an effective operator
\begin{equation}
    \mathcal{O} = \bar{\Psi} O \Psi\,,
\end{equation}
where $O$ is the meson factor composed of the meson, external sources, and derivatives, while the two nucleons $\Psi$ contract to it from two sides. The meson factor $O$ itself is of $(1/2,1/2)$ or $(0,0)$ representation of the Lorentz group and bi-fundamental representation of $SU(2)_V$, then one can construct all the meson factor $O$ of such representations. During such a process, covariant derivative $D_\mu$ is needed to apply to the nucleons sometimes so that the factor is of the required representations and does not change its power. For example, an order $\mathcal{O}(q^3)$ meson factor can be composed by two $u$ and one derivative $D$ on them, while only these building blocks can not form factors lying in the required representations, thus another derivative on nucleon is needed, thus there would be meson factors such as
\begin{equation}
   O^{(3)}_i = -\frac{1}{2m}[u_\mu,[D_\nu,u^\mu]]D^\nu + h.c.
\end{equation}
in Ref.~\cite{Fettes:2000gb}.

After careful comparison, we find we are in accordance with each other for some types such as $N^2u^2$, but for most types, our results are different.
Here we list the main differences as follows,
\begin{itemize}
    \item There are two operators obtained here that have no correspondence in Ref.~\cite{Fettes:2000gb} for both the relativistic and non-relativistic form, which are 
    \begin{equation}
        \bin{[D_\mu\tilde{f}_-{}^{\mu\nu},u_\nu]}\,,\quad  \bin{\gamma^\nu [u^\mu,f_-{}_{\mu\nu}]}\,.
    \end{equation}
    \item The effective operators are organized in terms of types in this paper. Because the derivatives on mesons or nucleons contribute differently to the power-counting, we move the derivatives from the nucleons using redundancy relations such as IBP as far as possible, and those that can not are attributed to lower power (those written in gray color in Sec.~\ref{sec:NMoperators}). While in Ref.~\cite{Fettes:2000gb}, the operators are organized strictly in terms of their power, and the derivatives are abused to form required representations, which means that the operators of different order may be not independent (usually are related by IBP). For example, there are three operators listed at $\mathcal{O}(q^4)$ order
    \begin{align}
        O^{(4)}_{33} & \rightarrow \bin{u_\mu}D^\mu\tra{\Sigma_-}\,,\notag \\
        O^{(4)}_{36} & \rightarrow \bin{}\tra{u_\mu D^\mu\Sigma_-}\,,\notag \\
        O^{(4)}_{37} & \rightarrow \bin{\sigma^{\mu\nu}[u_\mu,D_\nu \Sigma_-]}\,,
    \end{align}
    and an operator at $\mathcal{O}(q^3)$ of the same type
    \begin{equation}
        O^{(3)}_5 \rightarrow \bin{[\Sigma_-,u_\mu]\lrd^\mu}
    \end{equation}
    in Ref.~\cite{Fettes:2000gb}\footnote{Where we have recovered the nucleons to the meson factor and transferred them to our notation, $\chi\rightarrow \Sigma\,,\Psi\rightarrow N$.}. However, the operator $O^{(3)}_5$ is the same to $O^{(4)}_{37}$, which can be verified directly, 
    \begin{align}
        O^{(4)}_{37} &= -(D_\nu \overline{N}\sigma^{\mu\nu}[u_\mu,\Sigma_-]N) - (\overline{N}\sigma^{\mu\nu}[u_\mu,\Sigma_-]D_\nu N) - \underbrace{(\overline{N}\sigma^{\mu\nu}[D_\nu u_\mu,\Sigma_-]N)}_{=0} \notag \\
        & = -\frac{i}{2}(D_\nu \overline{N} \gamma^\mu\gamma^\nu [u_\mu,\Sigma_-] N) + \frac{i}{2}(\overline{N}\gamma^\nu\gamma^\mu[u_\mu,\Sigma_-] D_\nu N) 
        \quad \Leftarrow \text{EOM} \notag \\
        & = \frac{i}{2}( (\overline{N}\{\gamma^\nu,\gamma^\mu\} [u_\mu,\Sigma_-] D_\nu N) - (D_\nu \overline{N} \{\gamma^\mu,\gamma^\nu\} [u_\mu,\Sigma_-] N) ) 
        \quad \Leftarrow \text{EOM} \notag \\
        & = i ( (\overline{N} [u_\mu,\Sigma_-] D^\mu N) - (D^\mu \overline{N} [u_\mu,\Sigma_-] N) ) \quad \Leftarrow \{\gamma^\mu,\gamma^\nu\} = 2g^{\mu\nu} \notag \\
        & = i \bin{[\Sigma_-,u_\mu]\lrd^\mu} \notag \\
        & = i O^{(3)}_5\,.
    \end{align}
    \item In some type, Ref.~\cite{Fettes:2000gb} did not consider all the independent Lorentz or $SU(2)_V$ structures thus the relativistic effective operators there are not complete, but the non-relativistic form after HBP can be corresponded to the result here. For example, Ref.~\cite{Fettes:2000gb} only list two operators in type $N^2u^3$
    \begin{equation}
        O^{(3)}_{10} \rightarrow \bin{\gamma^5\gamma^\mu u_\mu}\lra{u_\nu u^\nu} \,,\quad O^{(3)}_{11} \rightarrow \bin{\gamma^5\gamma^\nu u^\mu}\lra{u_\nu u_\mu}
    \end{equation}
    and the operator $\bin{\gamma_\rho}\lra{[u_\mu,u_\nu]u_\sigma}\epsilon^{\mu\nu\rho\sigma}$ is missed since they did not consider the Lorentz structures containing tensor $\epsilon^{\mu\nu\rho\sigma}$. However, the operator $O^{(3)}_4$ in Ref.~\cite{Fettes:2000gb} has the same LO when doing HBP with the operator $\bin{\gamma_\rho}\lra{[u_\mu,u_\nu]u_\sigma}\epsilon^{\mu\nu\rho\sigma}$ presented here.
    \item Ref.~\cite{Fettes:2000gb} think $\tra{f_+}$ is an independent building block, but as seen in the definitions of $f^L$ and $f^R$ in Eq.~\ref{eq:fl} and Eq.~\ref{eq:fr} they are traceless since they are defined by commutators of covariant derivative. Thus, this paper has not presented the effective operators involving $\tra{f_+}$.
\end{itemize}

In summary, the cross-check of the Hilbert series and Young tensor method ensures that the operators presented in this paper are independent and complete. During the comparison with previous literature such as Ref.~\cite{Fettes:2000gb}, we find apart from some simple types, most of the operators there are redundant or not inadequate.




==> sec4-left.tex <==
\section{Chiral Symmetry for Low Energy EFT}
\label{sec:left}

Under the electro-weak scale, the physics is described by the low energy effective field theory (LEFT), which is though obtained from the SMEFT by integrating out the weak gauge bosons $W^\pm\,, Z$, the Higgs field $H$, and the top quark $t$, its generic effective Lagrangian itself deserves further research.


\subsection{Leading Order Lagrangian}

As an effective theory, the leading order of the LEFT Lagrangian is composed of QCD and QED parts,
\begin{align}
    \mathcal{L}_{LEFT,0} &= -\frac{1}{4} F_{\mu\nu}F^{\mu\nu} -\frac{1}{4}{G^A}_{\mu\nu}{G^A}^{\mu\nu} \notag \\
    &+\sum_{\psi=\mathbf{u}_L,\mathbf{u}_R} \bar{\psi}i\gamma^\mu D_\mu \psi + \sum_{\psi=,\mathbf{d}_L,\mathbf{d}_R} \bar{\psi}i\gamma^\mu D_\mu \psi +\sum_{\psi=,l_L,l_R,\nu_L} \bar{\psi}i\gamma^\mu D_\mu \psi \notag \\
    &-\sum_{\psi=u,d,e}(\bar{\psi}_L M_\psi \psi_R + h.c.) \,,
\end{align}
where the covariant derivative takes the form $D_\mu=\partial_\mu + ig T^AG^A_\mu + ie Q A_\mu$ with gluon field $G^A_\mu$ and photon field $A_\mu$.
The first line contains the dynamic terms of the photon and gluons\footnote{We do not consider strong CP term}, of which $F_{\mu\nu}$ is photon field-strength tensor and $G^A_{\mu\nu}$ is gluon field-strength tensor. The second line is dynamic terms of fermions, and the fermions are flavor multiplets
\begin{align}
    \mathbf{u}_{L/R} &= \left(\begin{array}{c}
u_{L/R} \\ c_{L/R}
    \end{array}\right) \,,\quad \mathbf{d}_{L/R} = \left(\begin{array}{c}
d_{L/R} \\ s_{L/R} \\b_{L/R}
    \end{array}\right)\,, \\
    l_{L/R} &= \left(\begin{array}{c}
e_{L/R} \\ \mu_{L/R} \\\tau_{L/R} 
    \end{array}\right) \,,\quad \nu_L = \left(\begin{array}{c}
{\nu_L}_e \\{\nu_L}_\mu \\ {\mu_L}_\tau 
\end{array}\right)\,.
\end{align}

The last line contains the mass terms of the fermions, in particular, the mass matrices $M_d\,, M_e$ are $3\times 3$ matrices while $M_u$ is $2\times 2$. In general, these mass matrices can be diagnosed by fermion field redefinition keeping the dynamic terms invariant.

For connection to the chiral operators, we can reformalize the quarks to form a certain representation of chiral symmetry $\mathcal{G}=SU(3)_L \times SU(3)_R$. To do that we join the up and down quarks together
\begin{equation}
    \textbf{q}_L = \left(\begin{array}{cccccc}
u_L & c_L & d_L & s_L & b_L 
    \end{array}\right)^T\,, \quad
    \textbf{q}_R = \left(\begin{array}{cccccc}
u_R & c_R & d_R & s_R & b_R 
    \end{array}\right)^T\,,
\end{equation}
then the mass term of quarks becomes $-\bar{\textbf{q}}_L \mathbf{M} \textbf{q}_R $ with
\begin{equation}
    \mathbf{M} = diag({m_u}\,, {m_c}\,,m_d\,,m_s\,,m_d)\,.
\end{equation}

If we reorganize the quark fields by the permutation matrix
\begin{equation}
    \mathbf{P}=\left(\begin{array}{ccccc}
1 & 0 & 0 & 0 & 0 \\ 0 & 0 & 1 & 0 & 0 \\ 0 & 0 & 0 & 1 & 0 \\ 0 & 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 & 1
    \end{array}\right)\,,
\end{equation}
the quark fields become
\begin{equation}
    \textbf{q}_{L/R} \rightarrow \mathbf{P} \textbf{q}_{L/R} = \textbf{q}_{L/R}^l \oplus \textbf{q}_{L/R}^h\,,
\end{equation}
where 
\begin{equation}
    \textbf{q}^l_{L/R} = \left(\begin{array}{ccc}
u_{L/R} & d_{L/R} & s_{L/R} 
    \end{array}\right)^T \,,\quad  \textbf{q}^h_{L/R} = \left(\begin{array}{ccc}
c_{L/R} & b_{L/R} 
    \end{array}\right)^T\,.
\end{equation} 
Thus the light and heavy quarks are separated, and their mass matrices are
\begin{equation}
    \textbf{M}_l = diag(m_u\,,u_d\,,m_s)\,,\quad \textbf{M}_h = diag(m_c\,,u_b)\,,
\end{equation}
with $\mathbf{P}^\dagger \mathbf{M}\mathbf{P}=\mathbf{M}_l \oplus \mathbf{M}_h$.
The light quarks are of irreducible representations of the chiral symmetry $SU(3)_L\times SU(3)_R$,
\begin{equation}
    \textbf{q}^l_L \in (\mathbf{3},\mathbf{1}) \,,\quad \textbf{q}^l_R \in (\mathbf{1},\mathbf{3})\,,
\end{equation}
while all other fields in the LEFT, including the heavy quark $\mathbf{q}_{L/R}^h$, leptons, and gauge bosons, are of trivial representation. 

In summary, the leading order Lagrangian of the LEFT can be expressed as $\mathcal{L}_{LEFT,0}=\mathcal{L}_{chiral}+\mathcal{L}_{current}$ with
\begin{align}
    \mathcal{L}_{chiral} &= \bar{\textbf{q}}^l_L i\gamma^\mu D_\mu \textbf{q}_L^l + \bar{\textbf{q}}^l_R i\gamma^\mu D_\mu \textbf{q}_R^l + (\bar{\textbf{q}}^l_L \mathbf{M}_l \textbf{q}_R^l + h.c.) \notag \\
    \mathcal{L}_{current} &=  -\frac{1}{4} F_{\mu\nu}F^{\mu\nu} -\frac{1}{4}{G^A}_{\mu\nu}{G^A}^{\mu\nu} + \sum_{\psi=l_L,l_R,\nu_L} \bar{\psi}i\gamma^\mu D_\mu \psi + \bar{\textbf{q}}^h_Li\gamma^\mu D_\mu \textbf{q}^h_L +  \bar{\textbf{q}}^h_Ri\gamma^\mu D_\mu \textbf{q}^h_R \notag \\
    &-(\bar{l}_L M_l l_R + \bar{\textbf{q}}^h_L \mathbf{M}_h \mathbf{q}^h_R + h.c.)\,.
\end{align}
In the ChEFT scenario, only the light quarks $\mathbf{q}^l_{L/R}$ can contribute to hadronic operators, and all the information of the heavy quarks $\mathbf{q}^h_{L/R}$ is buried in their coefficients. Besides, the other fields in the LEFT, such as the leptons and gauge bosons, can form external currents appearing in the hadronic operators. 


\subsection{Higher Order Operators}

From now on we consider the higher-order operators of the LEFT under chiral symmetry. As mentioned at the end of the last section, when corresponding to hadronic operators only the light quarks $\mathbf{q}^l_{L/R}$ are relevant, thus only the effective operators exclusive of the heavy quarks $\mathbf{q}^h_{L/R}$ are needed, so we let $\mathbf{q}_{L/R}$ denote the light quarks for simplicity in the subsequent discussion. In addition, since we do not discuss the isospin-violating operators in the ChEFT, the LEFT operators of interest should conserve the baryon number. 

Nevertheless, there are several obstructions when the chiral symmetry is extended to the higher order. The first problem is the construction of the irreducible representations of the chiral symmetry. Although it is challenging for the Young tensor method to form a non-trivial representation, the chiral symmetry, as a global symmetry, can be regarded as the extension of the flavor symmetry. It is usually the case the irreducible representation of the chiral symmetry is coincident with that of the flavor symmetry. For example, the dimension-6 effective operator $(\bar{\mathbf{q}}_R\mathbf{q}_L)(\bar{\mathbf{q}}_R \mathbf{q}_L)$ contain 2 repeated $\bar{\mathbf{q}}_R$ and two repeated $\mathbf{q}_L$. It is straightforward to see that the flavor structures of the two are simultaneously symmetric or anti-symmetric, thus the flavor irreducible representations are
\begin{equation}
    {\tiny\ydiagram{2}}\otimes {\tiny\ydiagram{2}} \oplus {\tiny\ydiagram{1,1}}\otimes {\tiny\ydiagram{1,1}}\,,
\end{equation}
corresponding to the $SU(n_f=3)$ irreducible representations
\begin{equation}
\label{eq:rep}
    \mathbf{6}\otimes \mathbf{6} \oplus \mathbf{3}\otimes \mathbf{3}\,.
\end{equation}
Noticing that $\bar{\mathbf{q}}_R$ is of the anti-fundamental representation of $SU(3)_R$, we can obtain the chiral symmetry representation
\begin{equation}
    (\mathbf{6},\bar{\mathbf{6}})\oplus (\bar{\mathbf{3}},\mathbf{3})\,.
\end{equation}
Apart from such a simple situation, there is another case where the irreducible flavor representations are not irreducible representations. In such a case, we need to do further tensor product decomposition. Considering the dimension operator $(\bar{\mathbf{q}}_L\gamma^\mu\mathbf{q}_L)(\bar{\mathbf{q}}_L\gamma_\mu\mathbf{q}_L)$, its flavor irreducible representation is the same with Eq.\ref{eq:rep}, but the corresponding chiral representation is reducible
\begin{equation}
    (\mathbf{6},\mathbf{1})\otimes (\bar{\mathbf{6}},\mathbf{1})\oplus(\mathbf{3},\mathbf{1})\otimes (\bar{\mathbf{3}},\mathbf{1})\,.
\end{equation}
After tensor product decomposition, we obtain the irreducible chiral representations that
\begin{equation}
    (\mathbf{27},\mathbf{1})\oplus 2\times (\mathbf{8},\mathbf{1})\oplus2\times(\mathbf{1},\mathbf{1})\,,
\end{equation}
where there are one $(\mathbf{27},\mathbf{1})$, two $(\mathbf{8},\mathbf{1})$ and two $(\mathbf{1},\mathbf{1})$\,. 

Another difficulty is electric charge conservation. In the LEFT, the electro-weak symmetry $SU(2)_{EW}\times U(1)_Y$ of the SMEFT breaks to the Abelian subgroup $U(1)_{em}$, representing electric charge conservation. When the light quarks are organized to form $SU(3)_{L/R}$ triplets. the electric charge conservation can be violated since the three light quarks take different charges
\begin{equation}
    \mathbf{q}_{L/R} = \left(
    \begin{array}{c}
u_{L/R} \sim \pm\frac{2}{3} \\ d_{L/R} \sim \mp \frac{1}{3} \\ s_{L/R} \sim \mp \frac{1}{3}
    \end{array}
    \right)\,.
\end{equation}
To recover the charge conservation, we need to write down the components explicitly. Considering the $(\mathbf{6},\bar{\mathbf{6}})$ representation of the dimension-6 operator  $(\bar{\mathbf{q}}_R\mathbf{q}_L)(\bar{\mathbf{q}}_R \mathbf{q}_L)$ again, there are 36 independent components, but not all of them conserve the electric charge. The SSYTs of the corresponding Young diagrams give a natural set of basis,
\begin{align}
    & \ytableaushort{11,22}\,,\quad \ytableaushort{11,33}\,,\quad \ytableaushort{22,33}\,,\quad \ytableaushort{12,23}\,,\quad \ytableaushort{12,33}\,,\quad \ytableaushort{11,23}\notag \\
    & \ytableaushort{12}\,,\quad \ytableaushort{13}\,,\quad \ytableaushort{23}\,,\quad \ytableaushort{11}\,,\quad \ytableaushort{22}\,,\quad \ytableaushort{33} \,.\label{eq:ssyts}
\end{align}
To relate these SSYTs to explicit operators, we define the tensor that
\begin{equation}
\label{eq:comp}
    \mathcal{O}_{xyyw|st}=(\bar{\mathbf{q}}_R^p\epsilon_{pxy}{\mathbf{q}_L}_s)(\bar{\mathbf{q}}_R^r\epsilon_{rvw} {\mathbf{q}_L}_t)\,,
\end{equation}
where $x,y,v,w$ are the $SU(3)_R$ indices, taking values of the indices in the $\bar{\mathbf{6}}$ representation
\begin{equation}
    {\tiny\ydiagram{2,2}}\,,
\end{equation}
$s,t$ are the $SU(3)_R$ indices, taking values of the indices in the $\bar{\mathbf{6}}$ representation
\begin{equation}
    {\tiny\ydiagram{2}}\,,
\end{equation}
and $\epsilon$ is the anti-symmetric tensor, so that an isomorphism between the operator components in Eq.~\ref{eq:comp} and the tensor products of the SSYTs in Eq.~\ref{eq:ssyts} via the application of the idempotent element on corresponding tensor. 
\begin{equation}
\label{eq:relation}
    \ytableaushort{ij,kl} \times \ytableaushort{mn} = \mathcal{Y}({\tiny\ytableaushort{13,24}})\times \mathcal{Y}({\tiny\ytableaushort{56}}) \mathcal{O}_{ijkl|mn}\,,
\end{equation}
where $\mathcal{Y}$ is the idempotent element of the corresponding standard Young tableaux
\begin{align}
    \mathcal{Y}({\tiny\ytableaushort{13,24}})&=\frac{1}{16}(1+(13))(1+(24))(1-(12))(1-(34)) \notag \\
    \mathcal{Y}({\tiny\ytableaushort{56}}) &= \frac{1}{2}(1+(56))\,,
\end{align}
and the permutation indices $1\sim 6$ is the order of the slots in the tensor $\mathcal{O}_{1234|56}$.
For example, the tensor product of the SSYTs
\begin{equation}
    \ytableaushort{11,22}\times \ytableaushort{23} 
\end{equation}
corresponds to the operator component
\begin{equation}
    \mathcal{Y}({\tiny\ytableaushort{13,24}})\times \mathcal{Y}({\tiny\ytableaushort{56}}) \mathcal{O}_{1212|23}\,,
\end{equation}
which can be simplified to a monomial
\begin{equation}
    \ytableaushort{11,22}\times \ytableaushort{23} = (\bar{\mathbf{q}}_R^3{\mathbf{q}_L}_2)(\bar{\mathbf{q}}_R^3 {\mathbf{q}_L}_3) = (\bar{s}_R d_L)(\bar{s}_R s_L)\,,
\end{equation}
which conserves electric charge and corresponds to the common LEFT operator $\mathcal{O}^{(4)}_{\bar{d}_R^2d_L^2}$. Similarly, we can get all 36 components and eliminate all the electric charge-violating ones. As a result, there are only 14 operators survive, which are presented in Tab~\ref{tab:example}.

\begin{table}[]
\renewcommand\arraystretch{1.5}
    \centering
    \begin{tabular}{c|c|c}
\hline
1 & \tiny\ytableaushort{11,22}$\times$\ytableaushort{23}  & $(\bar{s}_R  d_L)(\bar{s}_R  s_L)$\\
2 & \tiny\ytableaushort{12,23}$\times$\ytableaushort{12}  & $(\bar{s}_R  u_L)(\bar{u}_R  d_L)+(\bar{u}_R  u_L)(\bar{s}_R  d_L)$\\
3 & \tiny\ytableaushort{11,23}$\times$\ytableaushort{33}  & $(\bar{s}_R  d_L)(\bar{d}_R  d_L)$\\
4 & \tiny\ytableaushort{11,33}$\times$\ytableaushort{23}  & $(\bar{d}_R  d_L)(\bar{d}_R  s_L)$\\
5 & \tiny\ytableaushort{12,33}$\times$\ytableaushort{13}  & $(\bar{d}_R  u_L)(\bar{u}_R  s_L)+(\bar{u}_R  u_L)(\bar{d}_R  s_L)$\\
6 & \tiny\ytableaushort{11,23}$\times$\ytableaushort{33}  & $(\bar{s}_R  s_L)(\bar{d}_R  s_L)$\\
7 & \tiny\ytableaushort{11,22}$\times$\ytableaushort{22}  & $(\bar{s}_R  d_L)(\bar{s}_R  d_L)$\\
8 & \tiny\ytableaushort{11,33}$\times$\ytableaushort{33}  & $(\bar{d}_R  s_L)(\bar{d}_R  s_L)$\\
9 & \tiny\ytableaushort{11,22}$\times$\ytableaushort{33}  & $(\bar{s}_R  s_L)(\bar{s}_R  s_L)$\\
10 & \tiny\ytableaushort{11,33}$\times$\ytableaushort{22}  & $(\bar{d}_R  d_L)(\bar{d}_R  d_L)$\\
11 & \tiny\ytableaushort{22,33}$\times$\ytableaushort{11}  & $(\bar{u}_R  u_L)(\bar{u}_R  u_L)$\\
12 & \tiny\ytableaushort{12,23}$\times$\ytableaushort{13}  & $(\bar{s}_R  u_L)(\bar{u}_R  s_L)+(\bar{u}_R  u_L)(\bar{s}_R  s_L)$\\
13 & \tiny\ytableaushort{12,33}$\times$\ytableaushort{12}  & $(\bar{d}_R  u_L)(\bar{u}_R  d_L)+(\bar{u}_R  u_L)(\bar{d}_R  d_L)$\\
14 & \tiny\ytableaushort{11,23}$\times$\ytableaushort{23}  & $(\bar{s}_R  d_L)(\bar{d}_R  s_L)+(\bar{d}_R  d_L)(\bar{s}_R  s_L)$\\
\hline
    \end{tabular}
    \caption{The electric charge conservative operators from $(\bar{\mathbf{q}}_R\mathbf{q}_L)(\bar{\mathbf{q}}_R \mathbf{q}_L)$.}
    \label{tab:example}
\end{table}

It looks like it is awkward to exploit electric charge conservation under chiral symmetry since we need to write down and check all the components explicitly via the relations such as Eq.~\ref{eq:relation}, but keeping the compact form of certain chiral irreducible representation is still useful. On one hand, the check of electric charge conservation is not too tedious as it looks because of the important observation that in the triplet $\mathbf{q}_{L/R}$ the charge of the last two quarks,$d_{L/R},s_{L/R}$ are the same, and is opposite to the half of the charge of the first quark $u_{L/R}$. Thus the total number of $d_{L/R},s_{L/R}$ should be two times the number of $u_{L/R}$ to conserve the electric charge, which means that the frequencies of the indices $n_1,n_2$ and $n_3$ filled in the SSYTs should satisfy 
\begin{equation}
    n_1 = \frac{1}{3}N\,,\quad n_2+n_3 = \frac{1}{2}N\,,
\end{equation}
where $N$ is the number of total indices of the SSYT (just the number of boxes). It can be checked that all the SSYTs in Tab.~\ref{tab:example} satisfy this condition. More generally if the effective operators contain charged external current, the charge of the quark part is not zero, says $Q$, and the constraint becomes
\begin{equation}
    n_1 = \frac{1}{3}N + Q\,,\quad n_2+n_3 = \frac{1}{2}N - Q\,.
\end{equation}

On the other hand, the operators of chiral irreducible representations are convenient when corresponding to the hadronic operators, which will be discussed in a later discussion. To this end, we present the LEFT quark operators organized in terms of the chiral symmetry $\mathcal{G}$, in the explicit form of external currents separated in Tab.~\ref{tab:dim6}. The various external currents are defined as
\begin{equation}
\label{eq:current_1}
    j_{\psi_1\psi_2}^\pm = (\bar{\psi}_1\psi_2)\pm h.c.\,,\quad j_{\psi_1\psi_2}^{\pm\mu} = (\bar{\psi}_1\gamma^\mu\psi_2)\pm h.c.\,, \quad j_{\psi_1\psi_2}^{\pm \mu\nu} = (\bar{\psi}_1\sigma^{\mu\nu}\psi_2)\pm h.c.\,,
\end{equation}
\begin{align}
    & {j_{\psi_1\psi_2}^{D\pm\mu}} = (\overline{\psi}_1\overleftrightarrow{D}^\mu\psi_2)\pm h.c.\,,\quad {j_{\psi_1\psi_2}^{D\pm\mu\nu}} = (\overline{\psi}_1\gamma^\nu\overleftrightarrow{D}^\mu\psi_2)\pm h.c.\,,\notag \\ 
    & {j_{\psi_1\psi_2}^{D\pm\mu\nu\rho}} = (\overline{\psi}_1\sigma^{\nu\rho}\overleftrightarrow{D}^\mu\psi_2)\pm h.c.,\label{eq:current_2}
\end{align}
\begin{equation}
\label{eq:current_3}
    j_{X_1X_1} = {X_1}_{\mu\nu}{X_1}^{\mu\nu}\,,\quad j_{X_1X_2}^{\mu\nu}={X_1}^{\mu\rho}{X_2}^\nu_\rho\,,
\end{equation}
where $\psi_{1,2}$ is fermion and $X_{1,2}$ is gauge boson, $F$ or $\tilde F$.


\begin{table}[]
    \renewcommand{\arraystretch}{1}
        \centering
        \resizebox{\linewidth}{100mm}{ 
        \begin{tabular}{c|c|c|c|c}
    \hline
    \multirow{2}{*}{$\mathcal{G}$} & \multirow{2}{*}{Operator} & \multicolumn{3}{c}{$\chi$} \\
    \cline{3-5} 
    & & Lepton & Boson & combination \\
    \hline
    \multicolumn{5}{c}{ One quark current } \\
\hline
\multirow{6}{*}{$(\mathbf{3}\,\overline{\mathbf{3}})$}
& $(\overline{\mathbf{q}}_R\mathbf{q}_L)\chi$ 
& \makecell{$j_{\nu_L^c\nu_L}^{\pm}\,,j_{l_R\nu_L}^\pm\,,j_{l_L^c\nu_L}^\pm\,,$\\$j_{l_Rl_L}^\pm$} & $j_{FF}\,,j_{F\tilde{F}}\,,$ 
& \makecell{${j^{+\mu\nu}_{\nu_L^c\nu_L}}F_{\mu\nu}\,,{j^{-\mu\nu}_{\nu_L^c\nu_L}}\tilde{F}_{\mu\nu}\,,$ 
${j^{+\mu\nu}_{l_R\nu_L}}F_{\mu\nu}\,,{j^{-\mu\nu}_{l_R\nu_L}}\tilde{F}_{\mu\nu}\,,$ \\
${j^{+\mu\nu}_{l_L^c\nu_L}}F_{\mu\nu}\,,{j^{-\mu\nu}_{l_L^c\nu_L}}\tilde{F}_{\mu\nu}\,,$
${j^{+\mu\nu}_{l_R l_L}}F_{\mu\nu}\,,{j^{-\mu\nu}_{l_R l_L}}\tilde{F}_{\mu\nu}\,,$ } \\
\cline{2-5}
& $(\overline{\mathbf{q}}_R \overleftrightarrow{D}_\mu\mathbf{q}_L)\chi $ 
& \makecell{$j_{\nu_L\nu_L}^{+\mu}\,,j_{l_R^c\nu_L}^{\pm\mu}\,,j_{l_L\nu_L}^{\pm\mu}\,,$\\
$j_{l_Ll_L}^{+\mu}\,,j_{l_Rl_R}^{+\mu}$} 
& - & - \\
\cline{2-5}
& $(\overline{\mathbf{q}}_R\sigma_{\mu\nu}\mathbf{q}_L)\chi$ & $j_{l_R\nu_L}^{+\mu\nu}\,,j_{l_L^c\nu_L}^{+\mu\nu}\,,j_{l_R l_L}^{+\mu\nu}$ & - & 
\makecell{${j_{\nu_L^c\nu_L}^{\pm}} F^{\mu\nu}\,, {j_{\nu_L^c\nu_L}^{+\mu\rho}}F^\nu_\rho\,,$ 
${j_{l_R\nu_L}^{\pm}} F^{\mu\nu}\,, {j_{l_R\nu_L}^{+\mu\rho}}F^\nu_\rho\,,$ \\
${j_{l_L^c\nu_L}^{\pm}} F^{\mu\nu}\,, {j_{l_L^c\nu_L}^{+\mu\rho}}F^\nu_\rho\,,$ 
${j_{l_R l_L}^{\pm}} F^{\mu\nu}\,, {j_{l_R l_L}^{+\mu\rho}}F^\nu_\rho\,,$ } \\
\cline{2-5}
& $D^2(\overline{\mathbf{q}}_R \mathbf{q}_L)\chi$ 
& $j_{\nu_L^c\nu_L}^\pm\,,j_{l_R\nu_L}^\pm\,,j_{l_L^c\nu_L}^\pm\,,j_{l_Rl_L}^\pm$ & - & - \\
\cline{2-5}
& $D_\mu(\overline{\mathbf{q}}_R \overleftrightarrow{D}_\nu \mathbf{q}_L)\chi$ 
& $j_{\nu_L^c\nu_L}^{\pm\mu\nu}\,,j_{l_R\nu_L}^{\pm\mu\nu}\,,j_{l_L^c\nu_L}^{\pm\mu\nu}\,,j_{l_R l_L}^{\pm\mu\nu}$ & - & - \\
\cline{2-5}
& $(\overline{\mathbf{q}}_R\sigma_{\rho\lambda}\overleftrightarrow{D}_\mu\mathbf{q}_L)\chi$ 
& $ j_{\nu^c_L\nu_L}^{D+\mu\rho\lambda}\,,j_{l_R \nu_L}^{D+\mu\rho\lambda}\,,j_{l^c_L\nu_L}^{D+\mu\rho\lambda}\,,j_{l_R l_L}^{D+\mu\rho\lambda}$ & - & - \\
\hline
\multirow{6}{*}{$(\overline{\mathbf{3}}\,\mathbf{3})$} & $(\overline{\mathbf{q}}_L\mathbf{q}_R)\chi$ 
& \makecell{$j_{\nu_L^c\nu_L}^{\pm}\,,j_{l_R\nu_L}^\pm\,,j_{l_L^c\nu_L}^\pm\,,$\\$j_{l_Rl_L}^\pm$} & $j_{FF}\,,j_{F\tilde{F}}$ 
& \makecell{${j^{+\mu\nu}_{\nu_L^c\nu_L}}F_{\mu\nu}\,,{j^{-\mu\nu}_{\nu_L^c\nu_L}}\tilde{F}_{\mu\nu}\,,$ 
${j^{+\mu\nu}_{l_R\nu_L}}F_{\mu\nu}\,,{j^{-\mu\nu}_{l_R\nu_L}}\tilde{F}_{\mu\nu}\,,$ \\
${j^{+\mu\nu}_{l_L^c\nu_L}}F_{\mu\nu}\,,{j^{-\mu\nu}_{l_L^c\nu_L}}\tilde{F}_{\mu\nu}\,,$
${j^{+\mu\nu}_{l_R l_L}}F_{\mu\nu}\,,{j^{-\mu\nu}_{l_R l_L}}\tilde{F}_{\mu\nu}\,,$ } \\
\cline{2-5}
& $(\overline{\mathbf{q}}_L \overleftrightarrow{D}_\mu\mathbf{q}_R)\chi $ 
& \makecell{$j_{\nu_L\nu_L}^{+\mu}\,,j_{l_R^c\nu_L}^{\pm\mu}\,,j_{l_L\nu_L}^{\pm\mu}\,,$\\$j_{l_Ll_L}^{+\mu}\,,j_{l_Rl_R}^{+\mu}$} & - & -\\
\cline{2-5}
& $(\overline{\mathbf{q}}_L\sigma_{\mu\nu}\mathbf{q}_R)\chi$ & $j_{l_R\nu_L}^{+\mu\nu}\,,j_{l_L^c\nu_L}^{+\mu\nu}\,,j_{l_R l_L}^{+\mu\nu}$ & - & 
\makecell{${j_{\nu_L^c\nu_L}^{\pm}} F^{\mu\nu}\,, {j_{\nu_L^c\nu_L}^{+\mu\rho}}F^\nu_\rho\,,$ 
${j_{l_R\nu_L}^{\pm}} F^{\mu\nu}\,, {j_{l_R\nu_L}^{+\mu\rho}}F^\nu_\rho\,,$ \\
${j_{l_L^c\nu_L}^{\pm}} F^{\mu\nu}\,, {j_{l_L^c\nu_L}^{+\mu\rho}}F^\nu_\rho\,,$ 
${j_{l_R l_L}^{\pm}} F^{\mu\nu}\,, {j_{l_R l_L}^{+\mu\rho}}F^\nu_\rho\,,$ } \\
\cline{2-5}
& $D^2(\overline{\mathbf{q}}_L \mathbf{q}_R)\chi$ 
& $j_{\nu_L^c\nu_L}^\pm\,,j_{l_R\nu_L}^\pm\,,j_{l_L^c\nu_L}^\pm\,,j_{l_Rl_L}^\pm$ & - & - \\
\cline{2-5}
& $D_\mu(\overline{\mathbf{q}}_L \overleftrightarrow{D}_\nu \mathbf{q}_R)\chi$ 
& $j_{\nu_L^c\nu_L}^{\pm\mu\nu}\,,j_{l_R\nu_L}^{\pm\mu\nu}\,,j_{l_L^c\nu_L}^{\pm\mu\nu}\,,j_{l_R l_L}^{\pm\mu\nu}$ & - & - \\
\cline{2-5}
& $(\overline{\mathbf{q}}_L \sigma_{\rho\lambda}\overleftrightarrow{D}_\mu\mathbf{q}_R)\chi$ 
& $ j_{\nu^c_L\nu_L}^{D+\mu\rho\lambda}\,,j_{l_R \nu_L}^{D+\mu\rho\lambda}\,,j_{l^c_L\nu_L}^{D+\mu\rho\lambda}\,,j_{l_R l_L}^{D+\mu\rho\lambda}$ & - & - \\
\hline
\multirow{4}{*}{$(\mathbf{1},\mathbf{8})\oplus(\mathbf{1},\mathbf{1})$} 
& $(\overline{\mathbf{q}}_R\gamma_\mu \mathbf{q}_R)\chi$ 
& \makecell{${j_{\nu_L\nu_L}^{+\mu}}\,,{j_{l_R^c\nu_L}^{\pm\mu}}\,,{j_{l_L\nu_L}^{\pm\mu}}\,,$\\ 
${j_{l_L l_L}^{+\mu}}\,,{j_{l_R l_R}^{+\mu}}\,,{j_{l_Rl_L}^{D\pm\mu}}\,,$\\
${j_{\nu_L^c\nu_L}^{D\pm\mu}}\,,{j_{l_R\nu_L}^{D\pm\mu}}\,,{j_{l_L^c\nu_L}^{D\pm\mu}}$} & - 
& \makecell{$j_{\nu_L\nu_L}^{+\nu}F_\nu^\mu\,,j_{\nu_L\nu_L}^{+\nu}\tilde{F}_\nu^\mu\,, j_{l_R^c\nu_L}^{\pm\nu}F_\nu^\mu\,,j_{l_R^c\nu_L}^{\pm\nu}\tilde{F}_\nu^\mu\,,$\\
$j_{l_L\nu_L}^{\pm\nu}F_\nu^\mu\,,j_{l_L\nu_L}^{\pm\nu}\tilde{F}_\nu^\mu\,,j_{l_Rl_R}^{+\nu}F_\nu^\mu\,,j_{l_Rl_R}^{+\nu}\tilde{F}_\nu^\mu\,,$\\
$j_{l_Ll_L}^{+\nu}F_\nu^\mu\,,j_{l_Ll_L}^{+\nu}\tilde{F}_\nu^\mu$} \\
\cline{2-5}
& $(\overline{\mathbf{q}}_R\gamma_\mu \overleftrightarrow{D}_\nu \mathbf{q}_R)\chi$ & - 
& $j_{FF}^{\mu\nu}$ & - \\
\cline{2-5}
& $D^2(\overline{\mathbf{q}}_R\gamma_\nu \mathbf{q}_R)$ 
& $j_{\nu_L\nu_L}^{+\nu}\,,j_{l_L^c\nu_L}^{\pm\nu}\,,j_{l_L\nu_L}^{\pm\nu}\,,j_{l_R l_R}^{+\nu}\,,j_{l_L l_L}^{+\nu}$ & - & - \\
\cline{2-5}
& $(\overline{\mathbf{q}}_R\gamma_\mu \overleftrightarrow{D}_\nu\mathbf{q}_R)\chi$ 
& $ j_{\nu_L\nu_L}^{D+\mu\nu}\,,j_{l_L^c\nu_L}^{D\pm\mu\nu}\,,j_{l_L\nu_L}^{D\pm\mu\nu}\,,j_{l_R l_R}^{D+\mu\nu}\,,j_{l_L l_L}^{D+\mu\nu}$ & - & - \\
\hline
\multirow{4}{*}{$(\mathbf{8},\mathbf{1})\oplus(\mathbf{1},\mathbf{1})$} 
& $(\overline{\mathbf{q}}_L\gamma_\mu \mathbf{q}_L)\chi$ 
& \makecell{${j_{\nu_L\nu_L}^{+\mu}}\,,{j_{l_R^c\nu_L}^{\pm\mu}}\,,{j_{l_L\nu_L}^{\pm\mu}}\,,$\\ 
${j_{l_L l_L}^{+\mu}}\,,{j_{l_R l_R}^{+\mu}}\,,{j_{l_Rl_L}^{D\pm\mu}}\,,$\\
${j_{\nu_L^c\nu_L}^{D\pm\mu}}\,,{j_{l_R\nu_L}^{D\pm\mu}}\,,{j_{l_L^c\nu_L}^{D\pm\mu}}$} & - 
& \makecell{$j_{\nu_L\nu_L}^{+\nu}F_\nu^\mu\,,j_{\nu_L\nu_L}^{+\nu}\tilde{F}_\nu^\mu\,, j_{l_R^c\nu_L}^{\pm\nu}F_\nu^\mu\,,j_{l_R^c\nu_L}^{\pm\nu}\tilde{F}_\nu^\mu\,,$\\
$j_{l_L\nu_L}^{\pm\nu}F_\nu^\mu\,,j_{l_L\nu_L}^{\pm\nu}\tilde{F}_\nu^\mu\,,j_{l_Rl_R}^{+\nu}F_\nu^\mu\,,j_{l_Rl_R}^{+\nu}\tilde{F}_\nu^\mu\,,$\\
$j_{l_Ll_L}^{+\nu}F_\nu^\mu\,,j_{l_Ll_L}^{+\nu}\tilde{F}_\nu^\mu$} \\
\cline{2-5}
& $(\overline{\mathbf{q}}_L\gamma_\mu \overleftrightarrow{D}_\nu \mathbf{q}_L)\chi$ & - 
& $j_{FF}^{\mu\nu}$ & - \\
\cline{2-5}
& $D^2(\overline{\mathbf{q}}_L\gamma_\nu \mathbf{q}_L)$ 
& $j_{\nu_L\nu_L}^{+\nu}\,,j_{l_L^c\nu_L}^{\pm\nu}\,,j_{l_L\nu_L}^{\pm\nu}\,,j_{l_R l_R}^{+\nu}\,,j_{l_L l_L}^{+\nu}$ & - & - \\
\cline{2-5}
& $(\overline{\mathbf{q}}_L\gamma_\mu \overleftrightarrow{D}_\nu\mathbf{q}_L)\chi$ 
& $ j_{\nu_L\nu_L}^{D+\mu\nu}\,,j_{l_L^c\nu_L}^{D\pm\mu\nu}\,,j_{l_L\nu_L}^{D\pm\mu\nu}\,,j_{l_R l_R}^{D+\mu\nu}\,,j_{l_L l_L}^{D+\mu\nu}$ & - & - \\
\hline
        \end{tabular}
        }
        \caption{One-quark current operators of the LEFT organized by chiral symmetry. The external currents are defined in Eq.~\ref{eq:current_1}, Eq.~\ref{eq:current_2}, and Eq.~\ref{eq:current_3}.}
        \label{tab:dim6}
\end{table}

\begin{table}
    \renewcommand{\arraystretch}{1}
    \centering
    \resizebox{\linewidth}{100mm}{ 
    \begin{tabular}{c|c|c|c}
        \hline
        \multirow{2}{*}{$\mathcal{G}$} & \multirow{2}{*}{Operator} & \multicolumn{2}{c}{$\chi$} \\
        \cline{3-4} 
        & & Lepton & Boson  \\
        \hline
        \multicolumn{4}{c}{ Two quark currents (1) } \\
\hline
\multirow{6}{*}{$(\mathbf{6},\overline{\mathbf{6}})\oplus (\overline{\mathbf{3}},\mathbf{3})$} 
& $(\overline{\mathbf{q}}_R \mathbf{q}_L)(\overline{\mathbf{q}}_R \mathbf{q}_L)\chi $ 
& $j_{\nu_L^c\nu_L}^{\pm}\,,j_{l_R\nu_L}^{\pm}\,,j_{l_Rl_R^c}^{\pm}\,,j_{l_L^c \nu_L}^{\pm}\,,j_{l_Rl_L}^{\pm}\,,j_{l_L^c l_L}^{\pm}$ & 1 \\
\cline{2-4}
& $(\overline{\mathbf{q}}_R \sigma^{\mu\nu}\mathbf{q}_L)(\overline{\mathbf{q}}_R \sigma_{\mu\nu}\mathbf{q}_L)\chi$ 
& $j_{\nu_L^c\nu_L}^{\pm}\,,j_{l_R\nu_L}^{\pm}\,,j_{l_Rl_R^c}^{\pm}\,,j_{l_L^c \nu_L}^{\pm}\,,j_{l_Rl_L}^{\pm}\,,j_{l_L^c l_L}^{\pm}$ & 1 \\
\cline{2-4}
& $(\overline{\mathbf{q}}_R \mathbf{q}_L)D^2(\overline{\mathbf{q}}_R \mathbf{q}_L)\chi$ 
& - & 1 \\
\cline{2-4}
& $D_\mu(\overline{\mathbf{q}}_R \overleftrightarrow{D}_\nu\mathbf{q}_L)(\overline{\mathbf{q}}_R\sigma^{\mu\nu} \mathbf{q}_L)\chi$ 
& - & 1 \\
\cline{2-4}
& $(\overline{\mathbf{q}}_R\sigma^{\rho\lambda}\overleftrightarrow{D}^\mu \mathbf{q}_L)(\overline{\mathbf{q}}_R \sigma_{\rho\lambda}\overleftrightarrow{D}_\mu\mathbf{q}_L)\chi$ 
& - & 1 \\
\cline{2-4}
& $(\overline{\mathbf{q}}_R \sigma_{\mu\nu}\mathbf{q}_L)(\overline{\mathbf{q}}_R\mathbf{q}_L)\chi$ 
& $j_{\nu_L^c\nu_L}^{+\mu\nu}\,,j_{l_R \nu_L}^{+\mu\nu}\,,j_{l_R l_R^c}^{+\mu\nu}\,,j_{l_L^c \nu_L}^{+\mu\nu}\,,j_{l_R l_L}^{+\mu\nu}\,,j_{l_L^c l_L}^{+\mu\nu}$ & $F^{\mu\nu}$ \\
\hline
\multirow{2}{*}{$(\mathbf{6},\mathbf{3})\oplus(\overline{\mathbf{3}},\overline{\mathbf{6}})$} 
& $(\overline{\mathbf{q}}_R \sigma_{\mu\nu}\mathbf{q}_L)(\overline{\mathbf{q}}_R\mathbf{q}_L)\chi$ 
& $j_{\nu_L^c\nu_L}^{+\mu\nu}\,,j_{l_R \nu_L}^{+\mu\nu}\,,j_{l_R l_R^c}^{+\mu\nu}\,,j_{l_L^c \nu_L}^{+\mu\nu}\,,j_{l_R l_L}^{+\mu\nu}\,,j_{l_L^c l_L}^{+\mu\nu}$ 
& $F^{\mu\nu}$ \\
\cline{2-4}
& $(\overline{\mathbf{q}}_R\sigma_{\mu\rho}\mathbf{q}_L)(\overline{\mathbf{q}}_R\sigma^\rho_\nu \mathbf{q}_L)\chi$ 
& $j_{\nu_L^c\nu_L}^{+\mu\nu}\,,j_{l_R \nu_L}^{+\mu\nu}\,,j_{l_R l_R^c}^{+\mu\nu}\,,j_{l_L^c \nu_L}^{+\mu\nu}\,,j_{l_R l_L}^{+\mu\nu}\,,j_{l_L^c l_L}^{+\mu\nu}$ 
& $F^{\mu\nu}$ \\
\hline   
\multirow{6}{*}{$(\overline{\mathbf{6}},\mathbf{6})\oplus (\mathbf{3},\overline{\mathbf{3}})$} 
& $(\overline{\mathbf{q}}_L \mathbf{q}_R)(\overline{\mathbf{q}}_L \mathbf{q}_R)\chi $ 
& $j_{\nu_L^c\nu_L}^{\pm}\,,j_{l_R\nu_L}^{\pm}\,,j_{l_Rl_R^c}^{\pm}\,,j_{l_L^c \nu_L}^{\pm}\,,j_{l_Rl_L}^{\pm}\,,j_{l_L^c l_L}^{\pm}$ & 1 \\
\cline{2-4}
& $(\overline{\mathbf{q}}_L \sigma^{\mu\nu}\mathbf{q}_R)(\overline{\mathbf{q}}_L \sigma_{\mu\nu}\mathbf{q}_R)\chi$ 
& $j_{\nu_L^c\nu_L}^{\pm}\,,j_{l_R\nu_L}^{\pm}\,,j_{l_Rl_R^c}^{\pm}\,,j_{l_L^c \nu_L}^{\pm}\,,j_{l_Rl_L}^{\pm}\,,j_{l_L^c l_L}^{\pm}$ & 1 \\
\cline{2-4}
& $(\overline{\mathbf{q}}_L \mathbf{q}_R)D^2(\overline{\mathbf{q}}_L \mathbf{q}_R)\chi$ 
& - & 1 \\
\cline{2-4}
& $D_\mu(\overline{\mathbf{q}}_L \overleftrightarrow{D}_\nu\mathbf{q}_R)(\overline{\mathbf{q}}_L\sigma^{\mu\nu} \mathbf{q}_R)\chi$ 
& - & 1 \\
\cline{2-4}
& $(\overline{\mathbf{q}}_L\sigma^{\rho\lambda}\overleftrightarrow{D}^\mu \mathbf{q}_R)(\overline{\mathbf{q}}_L \sigma_{\rho\lambda}\overleftrightarrow{D}_\mu\mathbf{q}_R)\chi$ 
& - & 1 \\
\cline{2-4}
& $(\overline{\mathbf{q}}_L \sigma_{\mu\nu}\mathbf{q}_R)(\overline{\mathbf{q}}_L\mathbf{q}_R)\chi$ 
& $j_{\nu_L^c\nu_L}^{+\mu\nu}\,,j_{l_R \nu_L}^{+\mu\nu}\,,j_{l_R l_R^c}^{+\mu\nu}\,,j_{l_L^c \nu_L}^{+\mu\nu}\,,j_{l_R l_L}^{+\mu\nu}\,,j_{l_L^c l_L}^{+\mu\nu}$ & $F^{\mu\nu}$ \\
\hline
\multirow{2}{*}{$(\overline{\mathbf{6}},\overline{\mathbf{\mathbf{3}}})\oplus(\mathbf{3},\mathbf{6})$} 
& $(\overline{\mathbf{q}}_L \sigma_{\mu\nu}\mathbf{q}_R)(\overline{\mathbf{q}}_L\mathbf{q}_R)\chi$ 
& $j_{\nu_L^c\nu_L}^{+\mu\nu}\,,j_{l_R \nu_L}^{+\mu\nu}\,,j_{l_R l_R^c}^{+\mu\nu}\,,j_{l_L^c \nu_L}^{+\mu\nu}\,,j_{l_R l_L}^{+\mu\nu}\,,j_{l_L^c l_L}^{+\mu\nu}$ 
& $F^{\mu\nu}$ \\
\cline{2-4}
& $(\overline{\mathbf{q}}_L\sigma_{\mu\rho}\mathbf{q}_R)(\overline{\mathbf{q}}_L\sigma^\rho_\nu \mathbf{q}_R)\chi$ 
& $j_{\nu_L^c\nu_L}^{+\mu\nu}\,,j_{l_R \nu_L}^{+\mu\nu}\,,j_{l_R l_R^c}^{+\mu\nu}\,,j_{l_L^c \nu_L}^{+\mu\nu}\,,j_{l_R l_L}^{+\mu\nu}\,,j_{l_L^c l_L}^{+\mu\nu}$ 
& $F^{\mu\nu}$ \\
\hline
\multirow{3}{*}{\makecell{$(\mathbf{1},\mathbf{27})\oplus 2\times (\mathbf{1},\mathbf{8})$\\$\oplus2\times(\mathbf{1},\mathbf{1})$}} 
& $(\overline{\mathbf{q}}_R\gamma^\mu\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma_\mu\mathbf{q}_R)\chi$ 
& $j_{\nu_L^c\nu_L}^{\pm}\,,j_{l_R\nu_L}^{\pm}\,,j_{l_Rl_R^c}^{\pm}\,,j_{l_L^c \nu_L}^{\pm}\,,j_{l_Rl_L}^{\pm}\,,j_{l_L^c l_L}^{\pm}$ 
& 1 \\
\cline{2-4}
& $D^2(\overline{\mathbf{q}}_R \gamma^\nu \mathbf{q}_R)(\overline{\mathbf{q}}_R \gamma_\nu \mathbf{q}_R)$ 
& - & 1 \\
\cline{2-4}
& $(\overline{\mathbf{q}}_R \gamma^\nu \overleftrightarrow{D}^\mu\mathbf{q}_R)(\overline{\mathbf{q}}_R \gamma_\mu\overleftrightarrow{D}_\nu \mathbf{q}_R)$ 
& - & 1 \\
\hline
\makecell{$(\mathbf{1},\mathbf{10})\oplus (\mathbf{1},\overline{\mathbf{10}})$\\
$\oplus 2\times (\mathbf{1},\mathbf{8})$} 
& $(\overline{\mathbf{q}}_R\gamma_\mu \mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma_\nu \mathbf{q}_R)\chi$ 
& $j_{\nu_L^c\nu_L}^{\pm\mu\nu}\,,j_{l_R \nu_L}^{\pm\mu\nu}\,,j_{l_R l_R^c}^{\pm\mu\nu}\,,j_{l_L^c \nu_L}^{\pm\mu\nu}\,,j_{l_R l_L}^{\pm\mu\nu}\,,j_{l_L^c l_L}^{\pm\mu\nu}$ 
& $F^{\mu\nu}\,,\tilde{F}^{\mu\nu}$ \\
\hline
\multirow{3}{*}{\makecell{$(\mathbf{27},\mathbf{1})\oplus 2\times (\mathbf{8},\mathbf{1})$\\$\oplus2\times(\mathbf{1},\mathbf{1})$}} 
& $(\overline{\mathbf{q}}_L\gamma^\mu\mathbf{q}_L)(\overline{\mathbf{q}}_L\gamma_\mu\mathbf{q}_L)\chi$ 
& $j_{\nu_L^c\nu_L}^{\pm}\,,j_{l_R\nu_L}^{\pm}\,,j_{l_Rl_R^c}^{\pm}\,,j_{l_L^c \nu_L}^{\pm}\,,j_{l_Rl_L}^{\pm}\,,j_{l_L^c l_L}^{\pm}$ 
& 1 \\
\cline{2-4}
& $D^2(\overline{\mathbf{q}}_L \gamma^\nu \mathbf{q}_L)(\overline{\mathbf{q}}_L \gamma_\nu \mathbf{q}_L)$ 
&  & 1 \\
\cline{2-4}
& $(\overline{\mathbf{q}}_L \gamma^\nu \overleftrightarrow{D}^\mu\mathbf{q}_L)(\overline{\mathbf{q}}_L \gamma_\mu\overleftrightarrow{D}_\nu \mathbf{q}_L)$ 
& & 1 \\
\hline
\makecell{$(\mathbf{10},\mathbf{1})\oplus (\overline{\mathbf{10}},\overline{\mathbf{1}})$\\$\oplus 2\times (\mathbf{8},\mathbf{1})$} & $(\overline{\mathbf{q}}_L\gamma_\mu \mathbf{q}_L)(\overline{\mathbf{q}}_L\gamma_\nu \mathbf{q}_L)\chi$ 
& $j_{\nu_L^c\nu_L}^{\pm\mu\nu}\,,j_{l_R \nu_L}^{\pm\mu\nu}\,,j_{l_R l_R^c}^{\pm\mu\nu}\,,j_{l_L^c \nu_L}^{\pm\mu\nu}\,,j_{l_R l_L}^{\pm\mu\nu}\,,j_{l_L^c l_L}^{\pm\mu\nu}$ 
& $F^{\mu\nu}\,,\tilde{F}^{\mu\nu}$ \\
\hline   
    \end{tabular}
    }
    \caption{Two-quark current operators (1) of the LEFT organized by chiral symmetry. The external currents are defined in Eq.~\ref{eq:current_1}, Eq.~\ref{eq:current_2}, and Eq.~\ref{eq:current_3}.}
    \label{tab:dim81}
\end{table}

\begin{table}
    \renewcommand{\arraystretch}{1}
    \centering
    \resizebox{\linewidth}{100mm}{ 
    \begin{tabular}{c|c|c|c}
        \hline
        \multirow{2}{*}{$\mathcal{G}$} & \multirow{2}{*}{Operator} & \multicolumn{2}{c}{$\chi$} \\
        \cline{3-4} 
        & & Lepton & Boson  \\
        \hline
        \multicolumn{4}{c}{ Two quark currents (2) } \\
\hline
\multirow{9}{*}{\makecell{$(\mathbf{8},\mathbf{8})\oplus(\mathbf{8},\mathbf{1})$
\\$\oplus(\mathbf{1},\mathbf{8})\oplus(\mathbf{1},\mathbf{1})$}} 
& $(\overline{\mathbf{q}}_R \mathbf{q}_L)(\overline{\mathbf{q}}_L \mathbf{q}_R)\chi$ 
& $j_{\nu_L^c\nu_L}^{\pm}\,,j_{l_R\nu_L}^{\pm}\,,j_{l_Rl_R^c}^{\pm}\,,j_{l_L^c \nu_L}^{\pm}\,,j_{l_Rl_L}^{\pm}\,,j_{l_L^c l_L}^{\pm}$ 
& 1 \\
\cline{2-4}
& $(\overline{\mathbf{q}}_L\gamma^\mu \mathbf{q}_L)(\overline{\mathbf{q}}_R\gamma_\mu\mathbf{q}_R)\chi$ 
& $j_{\nu_L^c\nu_L}^{\pm}\,,j_{l_R\nu_L}^{\pm}\,,j_{l_Rl_R^c}^{\pm}\,,j_{l_L^c \nu_L}^{\pm}\,,j_{l_Rl_L}^{\pm}\,,j_{l_L^c l_L}^{\pm}$ 
& 1 \\
\cline{2-4}
& $(\overline{\mathbf{q}}_R\sigma_{\mu\nu}\mathbf{q}_L)(\overline{\mathbf{q}}_L\mathbf{q}_R)\chi$ 
& $j_{\nu_L^c\nu_L}^{+\mu\nu}\,,j_{l_R \nu_L}^{+\mu\nu}\,,j_{l_R l_R^c}^{+\mu\nu}\,,j_{l_L^c \nu_L}^{+\mu\nu}\,,j_{l_R l_L}^{+\mu\nu}\,,j_{l_L^c l_L}^{+\mu\nu}$ 
& $F^{\mu\nu}$ \\
\cline{2-4}
& $(\overline{\mathbf{q}}_R\mathbf{q}_L)(\overline{\mathbf{q}}_L\sigma_{\mu\nu}\mathbf{q}_R)\chi$ 
& $j_{\nu_L^c\nu_L}^{-\mu\nu}\,,j_{l_R \nu_L}^{-\mu\nu}\,,j_{l_R l_R^c}^{-\mu\nu}\,,j_{l_L^c \nu_L}^{-\mu\nu}\,,j_{l_R l_L}^{-\mu\nu}\,,j_{l_L^c l_L}^{-\mu\nu}$ 
& $\tilde{F}^{\mu\nu}$ \\
\cline{2-4}
& $(\overline{\mathbf{q}}_R\gamma_\mu\mathbf{q}_L)(\overline{\mathbf{q}}_L\gamma_\nu\mathbf{q}_R)\chi$ 
& $j_{\nu_L^c\nu_L}^{\pm\mu\nu}\,,j_{l_R \nu_L}^{\pm\mu\nu}\,,j_{l_R l_R^c}^{\pm\mu\nu}\,,j_{l_L^c \nu_L}^{\pm\mu\nu}\,,j_{l_R l_L}^{\pm\mu\nu}\,,j_{l_L^c l_L}^{\pm\mu\nu}$ 
& $F^{\mu\nu}\,,\tilde{F}^{\mu\nu}$ \\
\cline{2-4}
& $(\overline{\mathbf{q}}_R\mathbf{q}_L)D^2(\overline{\mathbf{q}}_L\mathbf{q}_R)$ 
& - & 1 \\
\cline{2-4}
& $(\overline{\mathbf{q}}_R\sigma_{\mu\nu}\mathbf{q}_L)D^\mu(\overline{\mathbf{q}}_L\overleftrightarrow{D}^\nu\mathbf{q}_R)$ 
& - & 1 \\
\cline{2-4}
& $D^2(\overline{\mathbf{q}}_R\gamma_\nu \mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma^\nu \mathbf{q}_R)$ 
& - & 1 \\
\cline{2-4}
& $(\overline{\mathbf{q}}_R\gamma_\nu\overleftrightarrow{D}_\mu \mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma^\mu\overleftrightarrow{D}^\nu \mathbf{q}_R)$ 
& - & 1 \\
\hline
\multirow{3}{*}{\makecell{$(\overline{\mathbf{10}},\overline{\mathbf{3}})\oplus(\mathbf{8},\overline{\mathbf{3}})$\\
$(\overline{\mathbf{6}},\overline{\mathbf{3}})\oplus(\mathbf{3},\overline{\mathbf{3}})$}}
& $(\overline{\mathbf{q}}_L\gamma^\mu \mathbf{q}_L)(\overline{\mathbf{q}}_R\overleftrightarrow{D}_\mu \mathbf{q}_L)\chi$ 
& - & 1 \\
\cline{2-4}
& $(\overline{\mathbf{q}}_L\gamma_\mu\mathbf{q}_L)(\overline{\mathbf{q}}_R\mathbf{q}_L)\chi$ 
& \makecell{$j_{\nu_L\nu_L}^{+\mu}\,,j_{l_R^c\nu_L}^{\pm\mu}\,,j_{l_L\nu_L}^{\pm\mu}\,,j_{l_R\nu_L^c}^{\pm\mu}\,,j_{l_R l_R}^{+\mu}\,,$\\
$j_{l_R l_L^c}^{\pm\mu}\,,j_{\nu_L l_L}^{\pm\mu}\,,j_{l_R^c l_L}^{\pm\mu}\,,j_{l_L;_L}^{\pm\mu}$} 
& - \\
\cline{2-4}
& $(\overline{\mathbf{q}}_L\gamma^\mu\mathbf{q}_L)(\overline{\mathbf{q}}_R\sigma_{\mu\nu}\mathbf{q}_L)\chi$ 
& \makecell{$j_{\nu_L\nu_L}^{+\nu}\,,j_{l_R^c\nu_L}^{\pm\nu}\,,j_{l_L\nu_L}^{\pm\nu}\,,j_{l_R\nu_L^c}^{\pm\nu}\,,j_{l_R l_R}^{+\nu}\,,$\\
$j_{l_R l_L^c}^{\pm\nu}\,,j_{\nu_L l_L}^{\pm\nu}\,,j_{l_R^c l_L}^{\pm\nu}\,,j_{l_L;_L}^{\pm\nu}$}
& - \\
\hline
\multirow{3}{*}{\makecell{$(\mathbf{10},\mathbf{3})\oplus(\mathbf{8},\mathbf{3})$\\
$\oplus(\mathbf{6},\mathbf{3})\oplus(\overline{\mathbf{3}},\mathbf{3})$}}
& $(\overline{\mathbf{q}}_L\gamma^\mu \mathbf{q}_L)(\overline{\mathbf{q}}_L\overleftrightarrow{D}_\mu \mathbf{q}_R)\chi$ 
& - & 1 \\
\cline{2-4}
& $(\overline{\mathbf{q}}_L\gamma_\mu\mathbf{q}_L)(\overline{\mathbf{q}}_L\mathbf{q}_R)\chi$ 
& \makecell{$j_{\nu_L\nu_L}^{+\mu}\,,j_{l_R^c\nu_L}^{\pm\mu}\,,j_{l_L\nu_L}^{\pm\mu}\,,j_{l_R\nu_L^c}^{\pm\mu}\,,j_{l_R l_R}^{+\mu}\,,$\\
$j_{l_R l_L^c}^{\pm\mu}\,,j_{\nu_L l_L}^{\pm\mu}\,,j_{l_R^c l_L}^{\pm\mu}\,,j_{l_L;_L}^{\pm\mu}$} 
& - \\
\cline{2-4}
& $(\overline{\mathbf{q}}_L\gamma^\mu\mathbf{q}_L)(\overline{\mathbf{q}}_L\sigma_{\mu\nu}\mathbf{q}_R)\chi$ 
& \makecell{$j_{\nu_L\nu_L}^{+\nu}\,,j_{l_R^c\nu_L}^{\pm\nu}\,,j_{l_L\nu_L}^{\pm\nu}\,,j_{l_R\nu_L^c}^{\pm\nu}\,,j_{l_R l_R}^{+\nu}\,,$\\
$j_{l_R l_L^c}^{\pm\nu}\,,j_{\nu_L l_L}^{\pm\nu}\,,j_{l_R^c l_L}^{\pm\nu}\,,j_{l_L;_L}^{\pm\nu}$}
& - \\
\hline
\multirow{3}{*}{\makecell{$(\mathbf{3},\mathbf{10})\oplus(\mathbf{3}.\mathbf{8})$\\
$\oplus(\mathbf{3}.\mathbf{6})\oplus(\mathbf{3},\overline{\mathbf{3}})$}} 
& $(\overline{\mathbf{q}}_R\gamma^\mu \mathbf{q}_R)(\overline{\mathbf{q}}_R\overleftrightarrow{D}_\mu \mathbf{q}_L)\chi$ 
& - & 1 \\
\cline{2-4}
& $(\overline{\mathbf{q}}_R\gamma_\mu\mathbf{q}_R)(\overline{\mathbf{q}}_R\mathbf{q}_L)\chi$ 
& \makecell{$j_{\nu_L\nu_L}^{+\mu}\,,j_{l_R^c\nu_L}^{\pm\mu}\,,j_{l_L\nu_L}^{\pm\mu}\,,j_{l_R\nu_L^c}^{\pm\mu}\,,j_{l_R l_R}^{+\mu}\,,$\\
$j_{l_R l_L^c}^{\pm\mu}\,,j_{\nu_L l_L}^{\pm\mu}\,,j_{l_R^c l_L}^{\pm\mu}\,,j_{l_L;_L}^{\pm\mu}$} 
& - \\
\cline{2-4}
& $(\overline{\mathbf{q}}_R\gamma^\mu\mathbf{q}_R)(\overline{\mathbf{q}}_R\sigma_{\mu\nu}\mathbf{q}_L)\chi$
& \makecell{$j_{\nu_L\nu_L}^{+\nu}\,,j_{l_R^c\nu_L}^{\pm\nu}\,,j_{l_L\nu_L}^{\pm\nu}\,,j_{l_R\nu_L^c}^{\pm\nu}\,,j_{l_R l_R}^{+\nu}\,,$\\
$j_{l_R l_L^c}^{\pm\nu}\,,j_{\nu_L l_L}^{\pm\nu}\,,j_{l_R^c l_L}^{\pm\nu}\,,j_{l_L;_L}^{\pm\nu}$} 
& - \\
\hline
\multirow{3}{*}{\makecell{$(\overline{\mathbf{3}},\overline{\mathbf{10}})\oplus(\overline{\mathbf{3}},\mathbf{8})$\\
$\oplus(\overline{\mathbf{3}},\overline{\mathbf{6}})\oplus(\overline{\mathbf{3}},\mathbf{3})$}} 
& $(\overline{\mathbf{q}}_R\gamma^\mu \mathbf{q}_R)(\overline{\mathbf{q}}_L\overleftrightarrow{D}_\mu \mathbf{q}_R)\chi$ 
& - & 1 \\
\cline{2-4}
& $(\overline{\mathbf{q}}_R\gamma_\mu\mathbf{q}_R)(\overline{\mathbf{q}}_L\mathbf{q}_R)\chi$ 
& \makecell{$j_{\nu_L\nu_L}^{+\mu}\,,j_{l_R^c\nu_L}^{\pm\mu}\,,j_{l_L\nu_L}^{\pm\mu}\,,j_{l_R\nu_L^c}^{\pm\mu}\,,j_{l_R l_R}^{+\mu}\,,$\\
$j_{l_R l_L^c}^{\pm\mu}\,,j_{\nu_L l_L}^{\pm\mu}\,,j_{l_R^c l_L}^{\pm\mu}\,,j_{l_L;_L}^{\pm\mu}$} 
& - \\
\cline{2-4}
& $(\overline{\mathbf{q}}_R\gamma^\mu\mathbf{q}_R)(\overline{\mathbf{q}}_L\sigma_{\mu\nu}\mathbf{q}_R)\chi$
& \makecell{$j_{\nu_L\nu_L}^{+\nu}\,,j_{l_R^c\nu_L}^{\pm\nu}\,,j_{l_L\nu_L}^{\pm\nu}\,,j_{l_R\nu_L^c}^{\pm\nu}\,,j_{l_R l_R}^{+\nu}\,,$\\
$j_{l_R l_L^c}^{\pm\nu}\,,j_{\nu_L l_L}^{\pm\nu}\,,j_{l_R^c l_L}^{\pm\nu}\,,j_{l_L;_L}^{\pm\nu}$} 
& - \\
\hline
    \end{tabular}
    }
    \caption{Two-quark current operators (2) of the LEFT organized by chiral symmetry. The external currents are defined in Eq.~\ref{eq:current_1}, Eq.~\ref{eq:current_2}, and Eq.~\ref{eq:current_3}.}
    \label{tab:dim82}
\end{table}

\begin{table}
    \renewcommand{\arraystretch}{2}
    \centering
    \resizebox{\linewidth}{100mm}{ 
    \begin{tabular}{c|c}
        \hline
        $\mathcal{G}$ & Operator($\chi=1$) \\
\hline
\multicolumn{2}{c}{ Three quark currents (1)} \\
\hline
$(\mathbf{10},\overline{\mathbf{10}})\oplus(\mathbf{1},\mathbf{1})$
& $(\overline{\mathbf{q}}_R\mathbf{q}_L)(\overline{\mathbf{q}}_R\mathbf{q}_L)(\overline{\mathbf{q}}_R\mathbf{q}_L)$,~
$(\overline{\mathbf{q}}_R\sigma^{\mu\nu}\mathbf{q}_L)(\overline{\mathbf{q}}_R\sigma_{\mu\nu}\mathbf{q}_L)(\overline{\mathbf{q}}_R\mathbf{q}_L)$ \\
\hline
\multirow{2}{*}{$(\mathbf{8},\mathbf{8})$}
& $(\overline{\mathbf{q}}_R\mathbf{q}_L)(\overline{\mathbf{q}}_R\mathbf{q}_L)(\overline{\mathbf{q}}_R\mathbf{q}_L)$,~
$(\overline{\mathbf{q}}_R\sigma^{\mu\nu}\mathbf{q}_L)(\overline{\mathbf{q}}_R\sigma_{\mu\nu}\mathbf{q}_L)(\overline{\mathbf{q}}_R\mathbf{q}_L)$,~
$(\overline{\mathbf{q}}_R\sigma^{\mu\nu}\mathbf{q}_L)(\overline{\mathbf{q}}_R\sigma_{\mu\rho}\mathbf{q}_L)(\overline{\mathbf{q}}_R\sigma^\rho_\nu\mathbf{q}_L)$ \\
& $(\overline{\mathbf{q}}_L\mathbf{q}_R)(\overline{\mathbf{q}}_L\mathbf{q}_R)(\overline{\mathbf{q}}_L\mathbf{q}_R)$,~
$(\overline{\mathbf{q}}_L\sigma^{\mu\nu}\mathbf{q}_R)(\overline{\mathbf{q}}_L\sigma_{\mu\nu}\mathbf{q}_R)(\overline{\mathbf{q}}_L\mathbf{q}_R)$,~
$(\overline{\mathbf{q}}_L\sigma^{\mu\nu}\mathbf{q}_R)(\overline{\mathbf{q}}_L\sigma_{\mu\rho}\mathbf{q}_R)(\overline{\mathbf{q}}_L\sigma^\rho_\nu\mathbf{q}_R)$ \\
\hline
\makecell{$(\mathbf{8},\mathbf{1})\oplus(\mathbf{1},\mathbf{8})$\\$\oplus(\mathbf{10},\mathbf{8})\oplus(\mathbf{8},\overline{\mathbf{10}})$\\$\oplus(\mathbf{10},\mathbf{1})\oplus(\mathbf{1},\overline{\mathbf{10}})$}
& $(\overline{\mathbf{q}}_R\sigma^{\mu\nu}\mathbf{q}_L)(\overline{\mathbf{q}}_R\sigma_{\mu\nu}\mathbf{q}_L)(\overline{\mathbf{q}}_R\mathbf{q}_L)$ \\
\hline
$(\mathbf{10},\overline{\mathbf{10}})\oplus(\mathbf{1},\mathbf{1})$
& $(\overline{\mathbf{q}}_L\mathbf{q}_R)(\overline{\mathbf{q}}_L\mathbf{q}_R)(\overline{\mathbf{q}}_L\mathbf{q}_R)$,~
$(\overline{\mathbf{q}}_L\sigma^{\mu\nu}\mathbf{q}_R)(\overline{\mathbf{q}}_L\sigma_{\mu\nu}\mathbf{q}_R)(\overline{\mathbf{q}}_L\mathbf{q}_R)$ \\
\hline
\makecell{$(\mathbf{8},\mathbf{1})\oplus(\mathbf{1},\mathbf{8})$\\$\oplus(\overline{\mathbf{10}},\mathbf{8})\oplus(\mathbf{8},\mathbf{10})$\\$\oplus(\overline{\mathbf{10}},\mathbf{1})\oplus(\mathbf{1},\mathbf{10})$}
& $(\overline{\mathbf{q}}_L\sigma^{\mu\nu}\mathbf{q}_R)(\overline{\mathbf{q}}_L\sigma_{\mu\nu}\mathbf{q}_R)(\overline{\mathbf{q}}_L\mathbf{q}_R)$ \\
\hline
\multirow{2}{*}{\makecell{$(\overline{\mathbf{10}},\mathbf{10})\oplus(\overline{\mathbf{10}},\mathbf{8})$\\
$\oplus(\mathbf{8},\mathbf{10})\oplus(\mathbf{8},\mathbf{8})$\\
$\oplus(\overline{\mathbf{6}},\mathbf{6})\oplus(\overline{\mathbf{6}},\overline{\mathbf{3}})$\\
$\oplus(\mathbf{3},\mathbf{6})\oplus(\mathbf{3},\overline{\mathbf{3}})$}}
& $(\overline{\mathbf{q}}_R\sigma^{\mu\nu}\mathbf{q}_L)(\overline{\mathbf{q}}_R\gamma_\mu\mathbf{q}_R)(\overline{\mathbf{q}}_L\gamma_\nu\mathbf{q}_L)$,~
$(\overline{\mathbf{q}}_R\mathbf{q}_L)(\overline{\mathbf{q}}_R\gamma_\mu\mathbf{q}_R)(\overline{\mathbf{q}}_L\gamma^\mu\mathbf{q}_L)$,~
$(\overline{\mathbf{q}}_R\mathbf{q}_L)(\overline{\mathbf{q}}_R\mathbf{q}_L)(\overline{\mathbf{q}}_L\mathbf{q}_R)$,~ \\
& $(\overline{\mathbf{q}}_R\sigma^{\mu\nu}\mathbf{q}_L)(\overline{\mathbf{q}}_R\sigma_{\mu\nu}\mathbf{q}_L)(\overline{\mathbf{q}}_L\mathbf{q}_R)$ \\
\hline
\makecell{$(\overline{\mathbf{6}},\mathbf{10})\oplus(\overline{\mathbf{6}},\mathbf{8})$\\
$\oplus(\mathbf{3},\mathbf{10})\oplus(\mathbf{3},\mathbf{8})$\\
$\oplus(\overline{\mathbf{10}},\mathbf{6})\oplus(\overline{\mathbf{10}},\overline{\mathbf{3}})$\\
$\oplus(\mathbf{8},\mathbf{6})\oplus(\mathbf{8},\overline{\mathbf{3}})$}
& $(\overline{\mathbf{q}}_R\sigma^{\mu\nu}\mathbf{q}_L)(\overline{\mathbf{q}}_R\gamma_\mu\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma_\nu\mathbf{q}_R)$,~
$(\overline{\mathbf{q}}_R\mathbf{q}_L)(\overline{\mathbf{q}}_R\gamma_\mu\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma^\mu\mathbf{q}_R)$ \\
\hline
\multirow{2}{*}{\makecell{$(\mathbf{10},\overline{\mathbf{10}})\oplus(\mathbf{10},\mathbf{8})$\\
$\oplus(\mathbf{8},\overline{\mathbf{10}})\oplus(\mathbf{8},\mathbf{8})$\\
$\oplus(\mathbf{6},\overline{\mathbf{6}})\oplus(\mathbf{6},\mathbf{3})$\\
$\oplus(\overline{\mathbf{3}},\overline{\mathbf{6}})\oplus(\overline{\mathbf{3}},\mathbf{3})$}}
& $(\overline{\mathbf{q}}_L\sigma^{\mu\nu}\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma_\mu\mathbf{q}_R)(\overline{\mathbf{q}}_L\gamma_\nu\mathbf{q}_L)$,~
$(\overline{\mathbf{q}}_L\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma_\mu\mathbf{q}_R)(\overline{\mathbf{q}}_L\gamma^\mu\mathbf{q}_L)$,~
$(\overline{\mathbf{q}}_L\mathbf{q}_R)(\overline{\mathbf{q}}_L\mathbf{q}_R)(\overline{\mathbf{q}}_R\mathbf{q}_L)$,~ \\
& $(\overline{\mathbf{q}}_L\sigma^{\mu\nu}\mathbf{q}_R)(\overline{\mathbf{q}}_L\sigma_{\mu\nu}\mathbf{q}_R)(\overline{\mathbf{q}}_R\mathbf{q}_L)$\\
\hline
\makecell{$(\mathbf{6},\overline{\mathbf{10}})\oplus(\mathbf{6},\mathbf{8})$\\
$\oplus(\overline{\mathbf{3}},\overline{\mathbf{10}})\oplus(\overline{\mathbf{3}},\mathbf{8})$\\
$\oplus(\mathbf{10},\overline{\mathbf{6}})\oplus(\mathbf{10},\mathbf{3})$\\
$\oplus(\mathbf{8},\overline{\mathbf{6}})\oplus(\mathbf{8},\mathbf{3})$}
& $(\overline{\mathbf{q}}_L\sigma^{\mu\nu}\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma_\mu\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma_\nu\mathbf{q}_R)$,~
$(\overline{\mathbf{q}}_L\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma_\mu\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma^\mu\mathbf{q}_R)$ \\
\hline
    \end{tabular}
    }
    \caption{Three-quark current operators (1) of the LEFT organized by chiral symmetry. The external currents are defined in Eq.~\ref{eq:current_1}, Eq.~\ref{eq:current_2}, and Eq.~\ref{eq:current_3}.}
    \label{tab:dim91}
\end{table}

\begin{table}
    \renewcommand{\arraystretch}{1}
    \centering
    \resizebox{\linewidth}{100mm}{ 
    \begin{tabular}{c|c}
        \hline
        $\mathcal{G}$ & Operator($\chi=1$) \\
\hline
\multicolumn{2}{c}{ Three quark currents (2)} \\
\hline
\makecell{$(\mathbf{3},\mathbf{21})\oplus(\mathbf{3},\mathbf{15})$\\$\oplus(\mathbf{3},\mathbf{24})\oplus(\mathbf{3},\overline{\mathbf{3}})$} & 
$(\overline{\mathbf{q}}_R\mathbf{q}_L)(\overline{\mathbf{q}}_R\gamma^\mu\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma_\mu\mathbf{q}_R)$ \\
\hline
$2\times (\mathbf{3},\overline{\mathbf{15}})\oplus (\mathbf{3},\mathbf{6})$ 
& $(\overline{\mathbf{q}}_R\sigma_{\mu\nu}\mathbf{q}_L)(\overline{\mathbf{q}}_R\gamma^\mu\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma^\nu\mathbf{q}_R)$ \\
\hline
\makecell{$(\mathbf{3},\mathbf{24})\oplus(\mathbf{3},\mathbf{15})$\\
$\oplus(\mathbf{3},\mathbf{6})\oplus(\mathbf{3},\mathbf{3})$\\
$\oplus(\mathbf{3},\overline{\mathbf{15}})\oplus(\mathbf{3},\overline{\mathbf{6}})$ \\
$\oplus(\mathbf{3},\overline{\mathbf{3}})$}
& $(\overline{\mathbf{q}}_R\mathbf{q}_L)(\overline{\mathbf{q}}_R\gamma_\mu\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma^\mu\mathbf{q}_R)$,~
$(\overline{\mathbf{q}}_R\sigma_{\mu\nu}\mathbf{q}_L)(\overline{\mathbf{q}}_R\gamma^\mu\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma^\nu\mathbf{q}_R)$ \\
\hline
\makecell{$(\mathbf{21},\mathbf{3})\oplus(\mathbf{15},\mathbf{3})$\\
$\oplus(\mathbf{24},\mathbf{3})\oplus(\overline{\mathbf{3}},\mathbf{3})$} & 
$(\overline{\mathbf{q}}_L\mathbf{q}_R)(\overline{\mathbf{q}}_L\gamma^\mu\mathbf{q}_L)(\overline{\mathbf{q}}_L\gamma_\mu\mathbf{q}_L)$ \\
\hline
$2\times (\overline{\mathbf{15}},\mathbf{3})\oplus (\mathbf{6},\mathbf{3})$ 
& $(\overline{\mathbf{q}}_L\sigma_{\mu\nu}\mathbf{q}_R)(\overline{\mathbf{q}}_L\gamma^\mu\mathbf{q}_L)(\overline{\mathbf{q}}_L\gamma^\nu\mathbf{q}_L)$ \\
\hline
\makecell{$(\mathbf{24},\mathbf{3})\oplus(\mathbf{15},\mathbf{3})$\\
$\oplus(\mathbf{6},\mathbf{3})\oplus(\mathbf{3},\mathbf{3})$\\
$\oplus(\overline{\mathbf{15}},\mathbf{3})\oplus(\overline{\mathbf{6}},\mathbf{3})$ \\
$\oplus(\overline{\mathbf{3}},\mathbf{3})$}
& $(\overline{\mathbf{q}}_L\mathbf{q}_R)(\overline{\mathbf{q}}_L\gamma_\mu\mathbf{q}_L)(\overline{\mathbf{q}}_L\gamma^\mu\mathbf{q}_L)$,~
$(\overline{\mathbf{q}}_L\sigma_{\mu\nu}\mathbf{q}_R)(\overline{\mathbf{q}}_L\gamma^\mu\mathbf{q}_L)(\overline{\mathbf{q}}_L\gamma^\nu\mathbf{q}_L)$ \\
\hline
\makecell{$(\overline{\mathbf{3}},\overline{\mathbf{21}})\oplus(\overline{\mathbf{3}},\overline{\mathbf{15}})$\\
$\oplus(\overline{\mathbf{3}},\overline{\mathbf{24}})\oplus(\overline{\mathbf{3}},\mathbf{3})$} & 
$(\overline{\mathbf{q}}_L\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma^\mu\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma_\mu\mathbf{q}_R)$ \\
\hline
$2\times (\overline{\mathbf{3}},\mathbf{15})\oplus (\overline{\mathbf{3}},\overline{\mathbf{6}})$ 
& $(\overline{\mathbf{q}}_L\sigma_{\mu\nu}\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma^\mu\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma^\nu\mathbf{q}_R)$ \\
\hline
\makecell{$(\overline{\mathbf{3}},\overline{\mathbf{24}})\oplus(\overline{\mathbf{3}},\overline{\mathbf{15}})$\\
$\oplus(\overline{\mathbf{3}},\overline{\mathbf{6}})\oplus(\overline{\mathbf{3}},\overline{\mathbf{3}})$\\
$\oplus(\overline{\mathbf{3}},\mathbf{15})\oplus(\overline{\mathbf{3}},\mathbf{6})$ \\
$\oplus(\overline{\mathbf{3}},\mathbf{3})$}
& $(\overline{\mathbf{q}}_L\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma_\mu\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma^\mu\mathbf{q}_R)$,~
$(\overline{\mathbf{q}}_L\sigma_{\mu\nu}\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma^\mu\mathbf{q}_R)(\overline{\mathbf{q}}_R\gamma^\nu\mathbf{q}_R)$ \\
\hline
\makecell{$(\overline{\mathbf{21}},\overline{\mathbf{3}})\oplus(\overline{\mathbf{15}},\overline{\mathbf{3}})$\\
$\oplus(\overline{\mathbf{24}},\overline{\mathbf{3}})\oplus(\mathbf{3},\overline{\mathbf{3}})$} & 
$(\overline{\mathbf{q}}_R\mathbf{q}_L)(\overline{\mathbf{q}}_L\gamma^\mu\mathbf{q}_L)(\overline{\mathbf{q}}_L\gamma_\mu\mathbf{q}_L)$ \\
\hline
$2\times (\mathbf{15},\overline{\mathbf{3}})\oplus (\overline{\mathbf{6}},\overline{\mathbf{3}})$ 
& $(\overline{\mathbf{q}}_R\sigma_{\mu\nu}\mathbf{q}_L)(\overline{\mathbf{q}}_L\gamma^\mu\mathbf{q}_L)(\overline{\mathbf{q}}_L\gamma^\nu\mathbf{q}_L)$ \\
\hline
\makecell{$(\overline{\mathbf{24}},\overline{\mathbf{3}})\oplus(\overline{\mathbf{15}},\overline{\mathbf{3}})$\\
$\oplus(\overline{\mathbf{6}},\overline{\mathbf{3}})\oplus(\overline{\mathbf{3}},\overline{\mathbf{3}})$\\
$\oplus(\mathbf{15},\overline{\mathbf{3}})\oplus(\mathbf{6},\overline{\mathbf{3}})$ \\
$\oplus(\mathbf{3},\overline{\mathbf{3}})$}
& $(\overline{\mathbf{q}}_R\mathbf{q}_L)(\overline{\mathbf{q}}_L\gamma_\mu\mathbf{q}_L)(\overline{\mathbf{q}}_L\gamma^\mu\mathbf{q}_L)$,~
$(\overline{\mathbf{q}}_R\sigma_{\mu\nu}\mathbf{q}_L)(\overline{\mathbf{q}}_L\gamma^\mu\mathbf{q}_L)(\overline{\mathbf{q}}_L\gamma^\nu\mathbf{q}_L)$ \\
\hline
    \end{tabular}
    }
    \caption{Three-quark current operators (2) of the LEFT organized by chiral symmetry. The external currents are defined in Eq.~\ref{eq:current_1}, Eq.~\ref{eq:current_2}, and Eq.~\ref{eq:current_3}.}
    \label{tab:dim6}
\end{table}

\iffalse
\begin{table}[]
    \centering
    \begin{tabular}{c|c|c}
\hline
Type & Operator & $SU(3)_L\times SU(3)_R$ \\
\hline
$\bar{\mathbf{q}}_R\mathbf{q}_L\bar{\nu}^c_L\nu_L+h.c.$ & $({\bar{\mathbf{q}}_R}{\mathbf{q}_L})({\bar{\nu}^c_L}{\nu_L})+ ({\bar{\mathbf{q}}_R}\sigma^{\mu\nu}{\mathbf{q}_L})({\bar{\nu}^c_L}\sigma_{\mu\nu}{\nu_L})$ & $(\mathbf{3},\bar{\mathbf{3}})$\\
\hline
\multirow{2}{*}{$\bar{\mathbf{q}}_R\mathbf{q}_L\bar{l}_R\nu_L+h.c.$} & $(\bar{\mathbf{q}}_R \mathbf{q}_L)(\bar{l}_R\nu_L)$ & \multirow{2}{*}{$(\mathbf{3},\bar{\mathbf{3}})$} \\
& $(\bar{\mathbf{q}}_R \sigma^{\mu\nu}\mathbf{q}_L)(\bar{l}_R\sigma_{\mu\nu}\nu_L)$ & \\
\hline
\multirow{2}{*}{$\bar{\mathbf{q}}_R\mathbf{q}_L\bar{l}^c_L\nu_L+h.c.$} & $(\bar{\mathbf{q}}_R \mathbf{q}_L)(\bar{l}_L^c\nu_L)$ & \multirow{2}{*}{$(\mathbf{3},\bar{\mathbf{3}})$} \\
& $(\bar{\mathbf{q}}_R \sigma^{\mu\nu}\mathbf{q}_L)(\bar{l}_L^c\sigma_{\mu\nu}\nu_L)$ & \\
\hline
\multirow{2}{*}{$\bar{\mathbf{q}}_R\mathbf{q}_L\bar{l}_R l_L+h.c.$} & $(\bar{\mathbf{q}}_R \mathbf{q}_L)(\bar{l}_R l_L)$ & \multirow{2}{*}{$(\mathbf{3},\bar{\mathbf{3}})$} \\
& $(\bar{\mathbf{q}}_R \sigma^{\mu\nu}\mathbf{q}_L)(\bar{l}_R\sigma_{\mu\nu} l_L)$ & \\
\hline
\multirow{2}{*}{${\bar{\mathbf{q}}_R}^2{\mathbf{q}_L}^2$} & $(\bar{\mathbf{q}}_R \mathbf{q}_L)(\bar{\mathbf{q}}_R \mathbf{q}_L)$ & \multirow{2}{*}{$(\mathbf{6},\bar{\mathbf{6}})\oplus (\bar{\mathbf{3}},\mathbf{3})$} \\
& $(\bar{\mathbf{q}}_R \sigma^{\mu\nu}\mathbf{q}_L)(\bar{\mathbf{q}}_R\sigma_{\mu\nu} \mathbf{q}_L)$ & \\
\hline
$\bar{\mathbf{q}}_L \mathbf{q}_R \bar{\nu}^c_L \nu_L$ & $(\bar{\mathbf{q}}_L \mathbf{q}_R)(\bar{\nu}_L^c \nu_L)$ & $(\bar{\mathbf{3}},\mathbf{3})$ \\
\hline
$\bar{\mathbf{q}}_L \mathbf{q}_R \bar{l}_R \nu_L$ & $(\bar{\mathbf{q}}_L \mathbf{q}_R)(\bar{l}_R\nu_L)$ & $(\bar{\mathbf{3}},\mathbf{3})$ \\
\hline
$\bar{\mathbf{q}}_L \mathbf{q}_R \bar{l}^c_L \nu_L$ & $(\bar{\mathbf{q}}_L \mathbf{q}_R)(\bar{l}_L^c \nu_L)$ & $(\bar{\mathbf{3}},\mathbf{3})$ \\
\hline
$\bar{\mathbf{q}}_L \mathbf{q}_R \bar{l}_R l_L$ & $(\bar{\mathbf{q}}_L \mathbf{q}_R)(\bar{l}_R l_L)$ & $(\bar{\mathbf{3}},\mathbf{3})$ \\
\hline
$\bar{\mathbf{q}}_R \mathbf{q}_R \bar{\nu}_L\nu_L$ & $(\bar{\mathbf{q}}_R\gamma^\mu \mathbf{q}_R)(\bar{\nu}_L\gamma_\mu \nu_L)$ & $(\mathbf{1},\mathbf{8})\oplus(\mathbf{1},\mathbf{1})$ \\
\hline
$\bar{\mathbf{q}}_R \mathbf{q}_R \bar{l}_R^c\nu_L$ & $(\bar{\mathbf{q}}_R\gamma^\mu \mathbf{q}_R)(\bar{l}_R^c\gamma_\mu \nu_L)$ & $(\mathbf{1},\mathbf{8})\oplus(\mathbf{1},\mathbf{1})$ \\
\hline
$\bar{\mathbf{q}}_R \mathbf{q}_R \bar{l}_L\nu_L$ & $(\bar{\mathbf{q}}_R\gamma^\mu \mathbf{q}_R)(\bar{l}_L\gamma_\mu \nu_L)$ & $(\mathbf{1},\mathbf{8})\oplus(\mathbf{1},\mathbf{1})$ \\
\hline
$\bar{\mathbf{q}}_R \mathbf{q}_R \bar{l}_R l_R$ & $(\bar{\mathbf{q}}_R\gamma^\mu \mathbf{q}_R)(\bar{l}_R\gamma_\mu l_R)$ & $(\mathbf{1},\mathbf{8})\oplus(\mathbf{1},\mathbf{1})$ \\
\hline
$\bar{\mathbf{q}}_R \mathbf{q}_R \bar{l}_Ll_L$ & $(\bar{\mathbf{q}}_R\gamma^\mu \mathbf{q}_R)(\bar{l}_L\gamma_\mu l_L)$ & $(\mathbf{1},\mathbf{8})\oplus(\mathbf{1},\mathbf{1})$ \\
\hline
$\bar{\mathbf{q}}_R^2\mathbf{q}_R^2$ & $(\bar{\mathbf{q}}_R\gamma^\mu\mathbf{q}_R)(\bar{\mathbf{q}}_R\gamma_\mu\mathbf{q}_R)$ & $(\mathbf{1},\mathbf{27})\oplus 2\times (\mathbf{1},\mathbf{8})\oplus2\times(\mathbf{1},\mathbf{1})$ \\
\hline
$\bar{\mathbf{q}}_L \mathbf{q}_L \bar{\nu}_L\nu_L$ & $(\bar{\mathbf{q}}_L\gamma^\mu \mathbf{q}_L)(\bar{\nu}_L\gamma_\mu \nu_L)$ & $(\mathbf{8},\mathbf{1})\oplus(\mathbf{1},\mathbf{1})$ \\
\hline
$\bar{\mathbf{q}}_L \mathbf{q}_L \bar{l}_R^c\nu_L$ & $(\bar{\mathbf{q}}_L\gamma^\mu \mathbf{q}_L)(\bar{l}_R^c\gamma_\mu \nu_L)$ & $(\mathbf{8},\mathbf{1})\oplus(\mathbf{1},\mathbf{1})$ \\
\hline
$\bar{\mathbf{q}}_L \mathbf{q}_L \bar{l}_L\nu_L$ & $(\bar{\mathbf{q}}_L\gamma^\mu \mathbf{q}_L)(\bar{l}_L\gamma_\mu \nu_L)$ & $(\mathbf{8},\mathbf{1})\oplus(\mathbf{1},\mathbf{1})$ \\
\hline
$\bar{\mathbf{q}}_L \mathbf{q}_L \bar{l}_R l_R$ & $(\bar{\mathbf{q}}_L\gamma^\mu \mathbf{q}_L)(\bar{l}_R\gamma_\mu l_R)$ & $(\mathbf{8},\mathbf{1})\oplus(\mathbf{1},\mathbf{1})$ \\
\hline
$\bar{\mathbf{q}}_L \mathbf{q}_L \bar{l}_Ll_L$ & $(\bar{\mathbf{q}}_L\gamma^\mu \mathbf{q}_L)(\bar{l}_L\gamma_\mu l_L)$ & $(\mathbf{8},\mathbf{1})\oplus(\mathbf{1},\mathbf{1})$ \\
\hline
$\bar{\mathbf{q}}_L^2\mathbf{q}_L^2$ & $(\bar{\mathbf{q}}_L\gamma^\mu\mathbf{q}_L)(\bar{\mathbf{q}}_L\gamma_\mu\mathbf{q}_L)$ & $(\mathbf{27},\mathbf{1})\oplus 2\times (\mathbf{8},\mathbf{1})\oplus2\times(\mathbf{1},\mathbf{1})$ \\
\hline
\multirow{2}{*}{$\bar{\mathbf{q}}_R\mathbf{q}_R\bar{\mathbf{q}}_L\mathbf{q}_L$} & $(\bar{\mathbf{q}}_R \mathbf{q}_L)(\bar{\mathbf{q}}_L \mathbf{q}_R)$ & \multirow{2}{*}{$(\mathbf{8},\mathbf{8})\oplus(\mathbf{8},\mathbf{1})\oplus(\mathbf{1},\mathbf{8})\oplus(\mathbf{1},\mathbf{1})$} \\
& $(\bar{\mathbf{q}}_L\gamma^\mu \mathbf{q}_L)(\bar{\mathbf{q}}_R\gamma_\mu\mathbf{q}_R)$ & \\
\hline
    \end{tabular}
    \caption{Dimension-6 operators contributing to hadronic operators}
    \label{tab:my_label}
\end{table}
\fi


%Only present quark level operators with SU(3) symmetry. 

%Reorganize the LEFT operators up to dim-8 (or dim-9) based on two-quark current, four-quark current, (six-quark current? not in  this work). 

%Separate 







==> sec8-weakcurrent.tex <==
\section{Weak Current Operator Bases}
\label{sec:weakoperator}


\subsection{Pure Meson Operators with Lepton Sources}

\subsection{Meson-Nucleon Operators with Lepton Sources}

\subsection{Nucleon-Nucleon Operators with Lepton Sources}

\subsection{Three Nucleon Operators with Lepton Sources}


%\subsection{Nuclear Potential from Chiral EFT}

%\subsection{Quark Level: LEFT Operators}
%
%\subsection{Nucleon Level: Pure Meson Operators}
%
%\subsection{Nucleon Level: Nucleon Meson Operators}
%
%\subsection{Nucleon Level: Nucleon Nucleon Operators}
%
%
%\subsection{Nuclear Potential from Chiral EFT}


